Unified Shape and SVBRDF Recovery using Differentiable Monte Carlo Rendering

Reconstructing the shape and appearance of real-world objects using measured 2D images has been a long-standing problem in computer vision. In this paper, we introduce a new analysis-by-synthesis technique capable of producing high-quality reconstructions through robust coarse-to-fine optimization and physics-based differentiable rendering. Unlike most previous methods that handle geometry and reflectance largely separately, our method unifies the optimization of both by leveraging image gradients with respect to both object reflectance and geometry. To obtain physically accurate gradient estimates, we develop a new GPU-based Monte Carlo differentiable renderer leveraging recent advances in differentiable rendering theory to offer unbiased gradients while enjoying better performance than existing tools like PyTorch3D and redner. To further improve robustness, we utilize several shape and material priors as well as a coarse-to-fine optimization strategy to reconstruct geometry. We demonstrate that our technique can produce reconstructions with higher quality than previous methods such as COLMAP and Kinect Fusion.

==> ablation.tex <==
\section{Ablation study}

==> comp1_fig.tex <==
\definecolor{lightgreen}{rgb}{0.388, 0.659, 0.447}
%
\begin{figure*}[p]
 \centering
    \setlength{\fboxsep}{0pt}%
    \setlength{\fboxrule}{0.5pt}%
    \contourlength{0.05em}%
    \vspace*{-0.1\baselineskip}%
    \hspace*{-2.0ex}%
    \begin{tikzpicture}[x=0.249\textwidth, y=0.249\textwidth,every text node part/.style={align=center}]
	    \node[anchor=north west] at (0,             0.67) {\includegraphics[width=0.166\textwidth]{results/compare1/cat/0000.jpg}};
	    \node[anchor=north west] at (0.667,         0.67) {\includegraphics[width=0.166\textwidth]{results/compare1/cat/0001.jpg}};
	    \node[anchor=north west] at (0.667*2,       0.67) {\includegraphics[width=0.166\textwidth]{results/compare1/cat/0002.jpg}};
	    \node[anchor=north west] at (0.667*3,       0.67) {\includegraphics[width=0.166\textwidth]{results/compare1/cat/0003.jpg}};
	    \node[anchor=north west] at (0.667*4,       0.67) {\includegraphics[width=0.166\textwidth]{results/compare1/cat/0004.jpg}};
	    \node[anchor=north west] at (0.667*5,       0.67) {\includegraphics[width=0.166\textwidth]{results/compare1/cat/0005.jpg}};
	
	
	    \node[anchor=north west] at (0,       0) {\includegraphics[width=0.248\textwidth]{results/compare1/sai_19_box.jpg}};
	    \node[anchor=north west] at (0+0.012,   -0.682 + 0.025) {\color{lightgreen}\fbox{\includegraphics[width=0.08\textwidth]{results/compare1/sai_19_zoom.jpg}}};
	    \node[anchor=north west] at (1,       0) {\includegraphics[width=0.248\textwidth]{results/compare1/nam_19_box.jpg}};
	    \node[anchor=north west] at (1+0.012,   -0.682 + 0.025) {\color{lightgreen}\fbox{\includegraphics[width=0.08\textwidth]{results/compare1/nam_19_zoom.jpg}}};
	    \node[anchor=north west] at (2,       0) {\includegraphics[width=0.248\textwidth]{results/compare1/our_19_warp_box.jpg}};
	    \node[anchor=north west] at (2+0.012,   -0.682 + 0.025) {\color{lightgreen}\fbox{\includegraphics[width=0.08\textwidth]{results/compare1/our_19_warp_zoom2.jpg}}};
	    \node[anchor=north west] at (3,       0) {\includegraphics[width=0.248\textwidth]{results/compare1/our_relit.jpg}};
	    
	
	    \node[anchor=north west] at (0,             -1.228) {\includegraphics[width=0.166\textwidth]{results/compare1/cactus/0000.jpg}};
	    \node[anchor=north west] at (0.667,         -1.228) {\includegraphics[width=0.166\textwidth]{results/compare1/cactus/0001.jpg}};
	    \node[anchor=north west] at (0.667*2,       -1.228) {\includegraphics[width=0.166\textwidth]{results/compare1/cactus/0002.jpg}};
	    \node[anchor=north west] at (0.667*3,       -1.228) {\includegraphics[width=0.166\textwidth]{results/compare1/cactus/0003.jpg}};
	    \node[anchor=north west] at (0.667*4,       -1.228) {\includegraphics[width=0.166\textwidth]{results/compare1/cactus/0004.jpg}};
	    \node[anchor=north west] at (0.667*5,       -1.228) {\includegraphics[width=0.166\textwidth]{results/compare1/cactus/0005.jpg}};
	    
	    \node[anchor=north west] at (0,       -1 - 0.9) {\includegraphics[width=0.248\textwidth]{results/compare1/sai_16_box.jpg}};
	    \node[anchor=north west] at (0+0.012,   -1.6785 + 0.025 - 0.9) {\color{lightgreen}\fbox{\includegraphics[width=0.08\textwidth]{results/compare1/sai_16_zoom.jpg}}};
	    \node[anchor=north west] at (1,       -1 - 0.9) {\includegraphics[width=0.248\textwidth]{results/compare1/nam_16_box.jpg}};
	    \node[anchor=north west] at (1+0.012,   -1.6785 + 0.025 - 0.9) {\color{lightgreen}\fbox{\includegraphics[width=0.08\textwidth]{results/compare1/nam_16_zoom.jpg}}};
	    \node[anchor=north west] at (2,       -1 - 0.9) {\includegraphics[width=0.248\textwidth]{results/compare1/our_16_box.jpg}};
	    \node[anchor=north west] at (2+0.012,   -1.6785 + 0.025 - 0.9) {\color{lightgreen}\fbox{\includegraphics[width=0.08\textwidth]{results/compare1/our_16_zoom.jpg}}};
	    \node[anchor=north west] at (3,       -1 - 0.9) {\includegraphics[width=0.248\textwidth]{results/compare1/our_relit2.jpg}};
	
	    \node[anchor=north west] at (1.65, 0.75)   {\textsc{\small Six photo inputs (Cat) }};
	    \node[anchor=north west] at (1.65, 0.75-1.91)   {\textsc{\small Six photo inputs (Cactus) }};
	
	    \node[anchor=north west] at (0+0.32,   -1.03) {\textsc{\scriptsize Bi et al.~\cite{bi2020deep}}};
	    \node[anchor=north west] at (1+0.32,   -1.03) {\textsc{\scriptsize Nam et al.~\cite{nam2018practical}}};
	    \node[anchor=north west] at (2+0.39,   -1.03) {\textsc{\scriptsize Ours}};
	    \node[anchor=north west] at (3+0.3,    -1.03) {\textsc{\scriptsize Ours (envmap)}};
	
	
	    \node[anchor=north west] at (0+0.32,   -3.03 + 0.1) {\textsc{\scriptsize Bi et al.~\cite{bi2020deep}}};
	    \node[anchor=north west] at (1+0.32,   -3.03 + 0.1) {\textsc{\scriptsize Nam et al.~\cite{nam2018practical}}};
	    \node[anchor=north west] at (2+0.39,   -3.03 + 0.1) {\textsc{\scriptsize Ours}};
	    \node[anchor=north west] at (3+0.3,    -3.03 + 0.1) {\textsc{\scriptsize Ours (envmap)}};
    \end{tikzpicture}%
    \vspace*{-0.1\baselineskip}%
    \caption{%
    	\small
    	Comparison with works by Bi et al.~\cite{bi2020deep} and Nam et al.~\cite{nam2018practical} on two real objects.
    	Using only 6 input images (shown in the top row of each example), Nam's method fails to recover the specular reflections, leading to visible artifacts in novel-view rendering (shown in the bottom row).
    	Bi's deep-learning-based technique is designed specifically for using such sparse inputs.
    	Our method manages to produce results that have quality on par with Bi's.
    	%produces results with comparable qualities under both novel-view point lighting and environmental illumination.
    }
    \label{fig:comp1}
\end{figure*}


==> envmap_fig.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.46\linewidth]{results2/envmap1.png} 
    \includegraphics[width=0.46\linewidth]{results2/chair_envmap.png}
    \includegraphics[width=0.46\linewidth]{results2/nefertiti_envmap.png}
    \includegraphics[width=0.46\linewidth]{results2/moai_envmap.png}
    \includegraphics[width=0.46\linewidth]{results2/egyptian-cat_envmap.png}
    \includegraphics[width=0.46\linewidth]{results2/metal-apple_envmap.png}
    \caption{Comparison of real and our recovered environment maps for the above five scenes: sofa, nefertiti, moai, egyptian cat and metal apple.}
    \label{fig:envmap}
\end{figure*}

==> failure_case.tex <==
\begin{figure*}[htp]
    \centering
    \setlength{\resLen}{1.6in}
    \addtolength{\tabcolsep}{-5pt}
    \small
    \begin{tabular}{cccc}
        \textsc{\scriptsize Init mesh} &
        \textsc{\scriptsize GT (point-light)} &
        \textsc{\scriptsize Ours (point-light)} &
        \textsc{\scriptsize Ours (normal)}\\
        \includegraphics[trim=75 75 75 75, clip,width=\resLen]{results/synthetic/buddha/KF.png} & 
        \includegraphics[trim=75 75 75 75, clip, width=\resLen]{results/synthetic/buddha/novel_tar.png} & 
        \includegraphics[trim=75 75 75 75, clip, width=\resLen]{results/synthetic/buddha/novel_fit.png} & 
        \includegraphics[trim=75 75 75 75, clip, width=\resLen]{results/synthetic/buddha/normal.png}\\
        \textsc{\scriptsize GT (env. map 1)} &
        \textsc{\scriptsize Ours (env. map 1)} &
        \textsc{\scriptsize GT (env. map 2)} &
        \textsc{\scriptsize Ours (env. map 2)}\\
        \includegraphics[trim=50 35 50 65, clip, width=\resLen]{results/synthetic/buddha/envmap1_tar.png} & 
        \includegraphics[trim=50 35 50 65, clip, width=\resLen]{results/synthetic/buddha/envmap1_fit.png} & 
        \includegraphics[trim=50 35 50 65, clip, width=\resLen]{results/synthetic/buddha/envmap2_tar.png} & 
        \includegraphics[trim=50 35 50 65, clip, width=\resLen]{results/synthetic/buddha/envmap2_fit.png}\\
    \end{tabular}
        \caption{Failure case. Given such a buddha model with complex geometry and highly glossy materials, our method is unable to accurately reproduce the appearance under novel uncontrolled illumination, even though we managed to optimize the geometric details back from a noisy and low-quality initial mesh. 
    \label{fig:failure}
\end{figure*}


==> method_initialization.tex <==
\subsection{Initialization}
\label{ssec:opt_init}
%
\begin{comment}
	\noindent\textbf{Geometry initialization.} Since our inverse rendering relies on gradient-based local optimization, we require a rough initial geometry to prevent severely large-scale mesh topology changes. From the captured images and camera poses, we first obtain a dense 3D point cloud using MVS~\cite{schoenberger2016mvs}. Due to the specular reflections created by our flash illumination which violates the underlying Lambertian shading assumption, this initial point cloud suffers from high-frequency noises. To address this, we use Poisson surface reconstruction~\cite{kazhdan2013screened, kazhdan2006poisson} to create a low-resolution mesh ($2^7$ voxel grid). When depth maps are available such as capturing with RGBD camera, we skip the COLMAP step and directly obtain an initial mesh from Kinect Fusion~\cite{newcombe2011kinectfusion}. After that, we additionally perform a follow-up topology fix to remove non-manifold edges, self-intersection triangles using MeshFix~\cite{attene2010lightweight}.\\ 
	
	\noindent\textbf{UV parameterization.} We globally parameterize the object mesh using iso-chart method~\cite{zhou2004iso, sawhney2017boundary} and represent surface points $x$ via their $(u, v)$ parametric coordinates in a rectangular image. Parameter space resolution is chosen manually, typically $1024 \times 1024$. In our coarse-to-fine framework, we progressively upsample the texture resolution, starting from $128\times 128$. One alternative representation is Mesh Color~\cite{yuksel2010mesh}, which was explored in prior work~\cite{bi2020deep, nam2018practical}. Comparing to storing SVBRDF parameters in the mesh directly as vertex colors, our PBR textures are directly reusable in graphics content pipeline such as a path tracer. \\ 
	
	\noindent\textbf{Roughness initialization.} We find that our method is robust to the initialization of material textures. We experimented with using the same initial configuration --- represented by the average RGB color over target images as constant diffuse map, a constant of $0.1$ as specular map and two constants of $0.5$ for the roughness initialization. However, this initialization represents a material with a high roughness (reflecting a bias for dielectric materials, as opposed to rough-conductor and metal materials) and sometimes lead to errors when fitting highly specular/low roughness materials. Therefore, we add an additional low initialization of $0.1$ constant roughness map. In practice, given the captured images, we run our optimization starting from both initialization and retain the result with the lowest optimization error. All of our results in this paper followed this scheme. A more complex initialization scheme is left as future work, such as using learning-based network predictions~\cite{li2018learning} as roughness initialization.
\end{comment}
%
Like any other analysis-by-synthesis method, our technique takes an input an initial configuration of an object's geometry and reflectance.
In theory, any initial configuration can be used, and our technique enjoys the robustness to work well even using initial configurations with very low quality (which we will demonstrate in \S\sz{XXX}).

In practice, we initialize object geometry in two ways.
When the object is measured using a simple handheld device such as a smartphone that has no depth-sensing capability, we obtain a dense 3D point cloud using multi-view stereo (MVS)~\cite{schoenberger2016mvs} and use Poisson surface reconstruction~\cite{kazhdan2013screened, kazhdan2006poisson} to create a low-resolution mesh.
On the other hand, when depth information is available, we directly obtain an initial mesh using Kinect Fusion~\cite{newcombe2011kinectfusion}.
We further post-process the intial meshes (provided by MVS or Kinect Fusion) to remove non-manifold edges and self-intersecting triangles using MeshFix~\cite{attene2010lightweight}.

Lastly, given an initial mesh, we generate per-vertex UV coordinates (that are needed to apply the reflectance textures) using  the iso-chart method~\cite{zhou2004iso, sawhney2017boundary}.


==> method_prelim.tex <==
\subsection{Acquisition Setup}
\label{ssec:setup}
%
Recent work has utilized collocated point illumination for reflectance estimation from a set of images captured on planar samples~\cite{aittala2015two, albert2018approximate, hui2017reflectance, riviere2016mobile, aittala2016reflectance, gao2019deep, deschaintre2019flexible, ren2011pocket}. Such lighting has the benefits of minimizing visible shadows in the captured photos and inducing strong high-frequency effects, leading to easier reflectance estimation. Similarly, this collocated point illumination setup has also been used in novel view synthesis~\cite{xu2019deep}, relighting~\cite{bi2020deepvol} and 3D capture~\cite{bi2020deep, nam2018practical, schmitt2020joint}. Motivated by this, we utilize a similar capture system --- a cellphone camera with flashlight, or a consumer-level handheld RGBD sensor with an LED light (see Figure~\ref{fig:setup}). In both cases, the point light is collocated with the camera location.


==> scan_fig.tex <==
 \begin{figure*}[t]
	\centering
	\setlength{\resLen}{0.385\columnwidth}
	%
   	\addtolength{\tabcolsep}{-5.4pt}
	\begin{tabular}{cc}
		\includegraphics[height=\resLen]{results/scan/ipad_lidar} &
		\includegraphics[height=\resLen]{results/scan/more_res_rabbit} \\ 
		{ (a) 3D scan using iPad.} &
		{ (b) High quality 3D model refinement using our pipeline.}
	\end{tabular}
    %
	\caption{\label{fig:app2}
		\textbf{Application:} Our pipeline can also facilitate low-cost LiDAR sensors (such as an iPad) and refine both the geometric details and SVBRDF textures.\zhao{the 2nd column of this image is a bit unclear to me, also should we show the mesh wireframe comparison between before and after optimization? we could remove one of the rendering results for more space. Also, note, this figure is not referenced in paper yet.}
	}
\end{figure*}





==> setup_fig.tex <==
\iffalse
	\begin{figure}[htp]
		\centering
	 
		\addtolength{\tabcolsep}{-4.5pt}
		\begin{tabular}{cc}
			{\scriptsize iPhone} & {\scriptsize Microsoft Azure Kinect}\\
			\includegraphics[height=1.65in]{setup/capture_iphone.jpg} &
			\includegraphics[height=1.65in]{setup/capture_sensor.jpg}
		\end{tabular}
		%
	    \caption{Multi-view acquisition setup. Our pipeline takes as input a set of photos captured by a collocated camera-light setup, which is commonly found on mobile phones or easily built on a consumer-level RGBD sensor, both with a collocated small LED light.}
	    \label{fig:setup}
	    %\vspace*{-1.5\baselineskip}%
	\end{figure}
\else
	\begin{center}
		\addtolength{\tabcolsep}{-4.5pt}
		\begin{tabular}{cc}
			{\scriptsize iPhone} & {\scriptsize Microsoft Azure Kinect}\\
			\includegraphics[height=1.65in]{setup/capture_iphone.jpg} &
			\includegraphics[height=1.65in]{setup/capture_sensor.jpg}
		\end{tabular}
	\end{center}
\fi


==> supp_setup.tex <==
\section{Acquisition setup}
\label{sec:setup}
%
To produce the reconstruction results of real-world objects in the paper and Figure~\ref{fig:main2_supp}, our method takes as input multi-view photos that can be captured using a camera with flashlight, or with a consumer-level RGBD sensor.
%In the later case, we can also utilize the depth information from RGBD sensor to accelarate the optimization process.
%
\input{setup_fig}


==> supp_tab_stages.tex <==
\begin{table}[htp]
	\centering
	\small
	\caption{\label{tab:supp_stages}
		\textbf{Number of stages and iterations per stage.} We report the number of stages in coarse-to-fine pipeline, and number of Adam iterations in each stage for both synthetic and real data.
	}
	\vspace{1em}
	\addtolength{\tabcolsep}{-3.5pt}
	\begin{tabular}{lcccccccc} 
		\toprule
		        &  Kitty & Duck & Bell & Pig  & Pony & Chime & Nefertiti & Buddha \\ 
		Stage 1 &  500   & 500  & 500  & 500  & 500  &  500  & 500       & 500    \\
		Stage 2 &  500   & 500  & 1000 & 1000 & 1000 & 1000  & 1000      & 1000   \\
		Stage 3 &  N/A   & N/A  & 500  & 500  & N/A  & 1000  & 1000      & 1000   \\
		Stage 4 &  N/A   & N/A  & N/A  & N/A  & N/A  &  500  & 500       & 500   \\
		\bottomrule
	\end{tabular}%
\end{table}


==> tab_geo_accuracy.tex <==
\begin{table}[b]
	\centering
	\small
	\caption{\label{tab:geo_accuracy}
		\textbf{Quantitative geometry evaluation}. We report the euclidean accuracy wrt. the ground truth geometry by computing the average point-to-mesh distance for all reconstructed points as described in \protect\cite{jensen2014large}.
	}
	\vspace{1em}
	\begin{tabular}{lcccc}
		\toprule
		& Pig & Bell & Duck & Kitty \\
		COLMAP               & 0.0017 & 0.0021 & 0.0135 & 0.0305\\
		Kinect Fusion (High) & 0.0149 & 0.0197 & 0.0079 & 0.0192\\
		Kinect Fusion (Low)  & 0.0318 & 0.0443 & 0.0353 & 0.0324\\
		Ours                 & \textbf{0.0006} & \textbf{0.0005} & \textbf{0.0011} & \textbf{0.0010}\\
		\bottomrule
	\end{tabular}
\end{table}

